LACO: A Latency-Driven Network Slicing Orchestration in Beyond-5G Networks

Network Slicing is expected to become a game changer in the upcoming 5G networks and beyond, enlarging the telecom business ecosystem through still-unexplored vertical industry profits. This implies that heterogeneous service level agreements (SLAs) must be guaranteed per slice given the multitude of predefined requirements. In this paper, we pioneer a novel radio slicing orchestration solution that simultaneously provides-latency and throughput guarantees in a multi-tenancy environment. Leveraging on a solid mathematical framework, we exploit the exploration-vs-exploitation paradigm by means of a multi-armed-bandit-based(MAB) orchestrator, LACO, that makes adaptive resource slicing decisions with no prior knowledge on the traffic demand or channel quality statistics. As opposed to traditional MAB methods that are blind to the underlying system, LACO relies on system structure information to expedite decisions. After a preliminary simulations campaign empirically proving the validness of our solution, we provide a robust implementation of LACO using off-the-shelf equipment to fully emulate realistic network conditions:near-optimal results within affordable computational time are measured when LACO is in place.

==> sections/POC.tex <==
 \begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{.33\textwidth}
      \includegraphics[trim = 14cm 0cm 1cm 1cm, clip, width=\linewidth ]{figures/Testbed_Final.pdf}
      \caption{Experimental setup.}
      \label{fig:testbed}
    \end{subfigure}%
    \begin{subfigure}[b]{.33\textwidth}
      \includegraphics[trim = 17cm 1.5cm 1.5cm 1.2cm, clip, width=\linewidth ]{figures/LACO_Architecture.pdf}
      \caption{Architecture overview.}
      \label{fig:architecture}
      \end{subfigure}%
    \begin{subfigure}[b]{.33\textwidth}
      \includegraphics[trim = 0cm 0cm 0cm 0cm, clip, width=\linewidth ]{figures/Arm_selection.pdf}
      \caption{Arm selection.}
      \label{fig:arm_selection}
      \end{subfigure}%
%  	\begin{subfigure}[b]{.25\textwidth}
%       \includegraphics[trim = 0cm 0cm 0cm 0cm, clip, width=\linewidth ]{figures/CDF_comparison.pdf}
%       \caption{CDF comparison.}
%       \label{fig:cdf_comparison}
%      \end{subfigure}
      \setlength{\abovecaptionskip}{-4pt} 
      \setlength{\belowcaptionskip}{-3pt} 
      \caption{\small Experimental setup (a); Architecture overview (b); Arm selection over time (c).}
    %   \caption{\small Experimental setup (a); Architecture overview (b); Arm selection over time (c) and comparison of slice delays (d).}
	\label{fig:POC_results}
	\vspace{-3mm}      
\end{figure*}

\section{Experimental Proof Of Concept}
\label{sect:poc}

In order to illustrate, validate and analyze the performance of our \name{} solution, we developed it as a standalone software module running on top of an open source platform that implements the LTE protocol stack, namely {\ttfamily srsLTE}~\cite{SRSLTE}, attached to a USRP\footnote{USRP B210 from National Instruments/Ettus Research (\url{https://www.ettus.com/all-products/UB210-KIT/}).} Software-Defined Radio (SDR) device as radio front-end. 
Our testbed is depicted in Fig.~\ref{fig:testbed} and consists of one LTE eNB (a modification of 
{\ttfamily srseNB}) and commercial Android tablets\footnote{Samsung Galaxy Tab S2 \url{ (https://www.samsung.com/de/tablets/galaxy-tab-s2-9-7-t813/SM-T813NZKEDBT/).}} as UEs. Any single UE emulates the aggregated traffic of multiple UEs within one slice. We use {\ttfamily mgen}\footnote{mgen (\url{https://www.nrl.navy.mil/itd/ncs/products/mgen}).} to generate different downlink traffic patterns.
Due to our LTE spectrum testing license restrictions, we use 10-MHz bandwidth in LTE band 7 and use SISO configuration for simplicity. This renders a maximum capacity of $\sim\!36$~Mb/s with highest SNR. Finally, in accordance with the findings described in \S\ref{sec:MAB_behaviour}, we set the minimum PRB allocation value at $10\%$ of the overall availability.

\subsection{Implementation}
The architecture of our software implementation and \name{}'s interfaces with {\ttfamily srseNB} are depicted in Fig.~\ref{fig:architecture}. \name{} interacts directly with the eNB's MAC layer to implement two key features:
\begin{itemize}
    \item {\bf Monitoring agent}. This feeds \name{} with real-time SNR reports generated by the PHY layer from feedback received from the UEs, the selected MCSs and corresponding transport block size (TBS) value used to encode information at the MAC layer, and other traffic statistics such as packet size and arrival times;
    \item {\bf Policy Enforcer}. This allows \name{} to dynamically enforce the PRB allocation policies calculated by our MAB model, as described in \S\ref{sect:mabmodel}.
\end{itemize}

The main feature of our implementation is the possibility to
collect, with TTI granularity, the traffic arrival rate and the TBS values to be used in each transmission frame. This information, together with the scheduling buffer size and data arrival times, is essential to compute the latency experienced by the different slices running in the system.

The different metrics are collected \edit{in a time series database, namely {\ttfamily InfluxDB}, and periodically reported to \name{} which constructs a virtual queue (one per slice) to track the dynamics of packets arriving at the eNB, from their entrance into the scheduling buffer to their transmission.}
This approach is particularly useful as IP packets are multiplexed while advancing the transmission path in the eNB, complicating the computation of slice latencies by external modules. Our approach aims to characterize the PRB allocation policy currently enforced into the system. In case of constant traffic and low latency requirements for example, poor channel conditions will result in lower TBS values and a sudden increase of the virtual queues size. Such event directly maps into an additional delay suffered by IP packets at the MAC layer.

Note that higher packet rates also lead to larger waiting times, which might result in exceeding slices SLAs boundaries. In such cases, the violation of pre-defined SLA latency boundaries triggers the DTMC model described in \S\ref{sect:MC} to a \emph{delay state} and the selected PRB allocation policy is assigned with a lower reward value.
Conversely, in a stable system where serving rate and packet arrival rate are balanced, the size of the virtual queues get smaller and the DTMC model is mostly characterized by \emph{non-delay states}.

%At first, we enabled connectivity between \name{} and the eNodeB scheduler opening sockets at Medium Access Control (MAC) layer (See Fig.~\ref{fig:architecture}). The advantage of this approach is two-fold, on the one side it allows to retrieve real-time (with TTI granularity) monitoring samples of multiple metrics e.g., SNR reports coming from PHY layer, MCS and corresponding TBS value, traffic statistics (for example packet size and time of arrival in the scheduler buffer), etc., which are crucial to estimate the latency experienced by the traffic flows. On the other side, it provides the means to reach the scheduling entity in the eNodeB and dynamically enforce the selected PRB allocation policy.
%In our setup the eNodeB instance runs on top of an Ettus USRP B$210$ RF front-end and operates at band $3$ with $10$ MHz channel bandwidth, which leads to an overall $50$ PRBs availability. In accordance with the findings described in \S\ref{sec:MAB_behaviour}, we set the minimum PRB allocation value at $10\%$ of this overall amount.
%We use commercial tablets to emulate slice users and open source traffic generators to mimic the traffic load offered by different network slices. In particular, each downlink flow reaching the devices represents the aggregated traffic generated by one slice.

\edit{

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{.5\textwidth}
      \includegraphics[trim = 0cm 0cm 0cm 0cm, clip, width=\linewidth ]{figures/Discovery_Phase.pdf}
      \caption{System dynamics during MAB discovery phase.}
      \label{fig:discovery_phase}
    \end{subfigure}%
    \begin{subfigure}[b]{.5\textwidth}
      \includegraphics[trim = 0cm 0cm 0cm 0cm, clip, width=\linewidth ]{figures/Final_Phase.pdf}
    \caption{System dynamics at convergence.}
    \label{fig:final_phase}
      \end{subfigure}%
      \caption{\small Comparison of system dynamics during a) discovery phase and b) MAB convergence.}
	\label{fig:MAB_Evolution}
	\vspace{-3mm}      
\end{figure*}

\subsection{Experimental results}
\tbd{Fix slice requirements}
We first consider a scenario with two slices with the following requirements. The first slice (labelled Ultra Reliable Low Latency Communications or URLLC) demands $\Delta_{\textit{URLLC}}\le5$~ms communication delay and is characterized by a constant bit rate equal to $8$~Mb/s. The second slice (labelled enhanced Mobile Broaband or eMBB) is characterized by the same throughput magnitude and distribution but a more relaxed latency requirements of $\Delta_{\textit{eMBB}}\le30$~ms. We set \name{}'s decision interval to $15$ seconds and let our experiment run for $100$ decision intervals. Fig.~\ref{fig:arm_selection} shows the evolution of the PRB allocation  configuration decisions taken by \name{} over this time span and how fast the convergence is achieved. 

As described in Sec.~\ref{sect:mabmodel}, during the starting procedure the MAB algorithm explores all the available arms, i.e. configurations, with the aim to collect an initial feedback on the system dynamics. Fig.~\ref{fig:discovery_phase} depicts the effects of such sequential choices on the latency experienced by the ongoing traffic flows. It can be noticed how the initial steps favour the allocation of radio resources to the eMBB slice, providing significant advantages in terms of latency with respect to the second one. The scenario inverts around the $4$-th decision interval, when the agent selects configurations which do not guarantee the allocation of enough resources to satisfy the latency requirements. Interestingly despite similar traffic requirements, the algorithm finally selects a configuration which assigns more resources to the first slice. This can be justified by the lower SNR value experienced by such slice, which thus requires more PRBs to compensate for the lower MCS used during the communication.


We further investigate the performance of \name{} and consider a more complicated scenario including $3$ slices.
The first, labelled as URLLC, characterized by \tbd{}.
The second, labelled as eMBB, characterized by random bursts of Poisson distributed traffic with peaks of $18$~Mb/s, average inter-burst time equal to $0.4$~s and burst duration exponentially distributed with mean equal to $0.8$~s. The third, labelled as \tbd{}, characterized by \tbd{}.

The latency performance results of our experiment are summarized in Fig.~\ref{fig:cdf_comparison}. The performance of the URLLC slice is shown on the left-side plot whereas the eMBB's one on the right-side plot: both plots depict the empirical CDF of the latency incurred when applying \name{} (in black) as well as {\ttfamily srsLTE}'s round-robin (RR) PRB allocation policy (in blue), used as the main benchmark. 

Based on these results we can observe that \name{} successfully meets both slices latency requirements as compared to RR which fails to do so. This is achieved by providing the required resources to the URLLC and eMBB slices (Fig.~\ref{fig:arm_selection}) according to their different latency needs. This results in the URLLC slice meeting the SLA latency requirements (<5ms) at a very low latency cost increase for the eMBB slice. In our experiments, only $2\%$ of the traffic experienced a latency above the $5$~ms target of URLLC when using \name{}, in contrast to the $46\%$ experienced with RR. Note that this $2\%$ is due to the \name{} solution convergence period. Thus, the longer the lifetime of the URLLC network slice, the lower the probability of experiencing a latency above the SLA. %; and  $3\%$ and $5\%$, respectively, of traffic violating the $30$~ms target for the eMBB slice.


}

%\edit{
%This is further confirmed by Fig.~\ref{fig:cdf_comparison}, which yields an insight of the latency experienced by the single packets as results of the monitoring activities performed at the scheduling buffer during the experiment. It can be noticed that in presence of \name{} an additional $50\%$ of the traffic meets the latency requirements of the URLLC slice when compared to legacy round-robin scheduling.
%It is expected that to guarantee the latency targets of the first slice, the eMBB slice will suffer worst performance. However, our measurements show that this gap of performance is negligible and still enclosed within the bounds defined by the latency requirements of the slice.
%}

==> sections/PerformanceEvaluation.tex <==
\section{Performance Evaluation}
\label{sect:perf_eval}

%We evaluate our solution through an exhaustive simulation campaign that implements the Multi-Armed Bandit problem in the context of radio resource allocation of network slices.

%where the incoming rewards, obtained as defined in \S\ref{sect:reward_def}, shape the decision process. 
%We evaluate the performance of our solution in terms of aggregate reward and cumulative latency.
%mapping the network slice radio resource allocation decision into a MAB problem where each arm represents a possible resource assignment, and the reward is a measure of the latency experienced by the slice with that configuration, namely, the higher reward, the lower the latency. 

%Therefore, we associate each tenant with a predefined class that includes a network slice type, based on the network slice templates (NST)~\cite{XX} that the infrastructure provider may offer to the tenants.

%Therefore, we simulate the traffic generated by each slice as a random variable derived by different Gaussian distribution $\mathcal{N}(\mu ,\nu^2 )$ characterized by mean $\mu$ and standard deviation $\nu$ as reported in Table~\ref{tab:slices}.

In this section, we evaluate our solution through an exhaustive simulation campaign that takes into account complexity, revenue and SLA violation metrics. 
%Tenants may present heterogeneous requirements in terms of traffic demand and SLAs~\cite{Slicing2018CoNEXT}. Therefore, we derive the traffic generated by the $i$-th slice from a Normal distribution $\mathcal{N}_i (\mu_i ,\nu_i^2 )$ bits per second, where $\mu_i$ and $\nu_i$ represent the mean value and standard deviation, respectively, and $L_i$ accounts for the latency constraint latency requirements. 

\subsection{Simulations setup}
To assess heterogeneous slices, we simulate the network load demand of slice $i$ at each time-slot (i.e., each transmission time interval (TTI) in LTE systems) by extracting a random value from a Normal distribution $\mathcal{N}_i (\mu_i ,\nu_i^2 )$, where $\mu_i$ and $\nu_i$ represent the mean value and standard deviation, and let $L_i$ describe its latency constraint.

%As explained earlier, each resource assignment (or arm) is associated with a set of Markov chains providing information about the latency experienced with that setup. 
Moreover, we model the SNR channel variation as another random variable drawn by a Rayleigh distribution and derive the probability distribution encompassing the whole SNR range.
%We upper-bound this range with $\textit{SNR}_{MAX}=40$ dB.
For every channel instantiation, we extract the corresponding Modulation and Coding Scheme (MCS) as defined by the 3GPP standard.\footnote{We refer the reader to~\cite{TS36.213} for an exhaustive explanation of the mapping between SNR and MCS.} The MCS index $m \in \mathcal{M}$ combines one possible modulation scheme and a predefined coding rate providing a compact way to represent a simple concept: the better the radio conditions, the more bits can be transmitted per time unit, and \emph{vice versa}. 
Fixing the channel bandwidth at $20$ MHz,
conventional value in LTE systems, the expected average throughput achievable by one slice during one epoch depends on both the modulation and coding schemes used and, most importantly, on the number of PRBs reserved for the slice. In a wider timescale\,\footnote{Note that we assume a timescale larger than our epochs used in the decision-making process.}, the average capacity can be approximated as $C_i = \left( \sum_{m}^{M} \Gamma_{m} \pi_{m,i} \right) T_i y_i$ where $\Gamma_{m}$ represents the average number of bits per LTE subframe that can be transmitted using the $m$-th MCS index, $\pi_{m,i}$ is the steady-state probability distribution output of the first stage Markov chain model, $T_i$ defines the decision interval size, and $y_i$ accounts for the number of PRBs allocated to the $i$-th slice. We refer the reader to Table~\ref{tab:notations}.

%the number of spatial streams to use in the transmission (MIMO technology), the MCS index and the transmission block size, it is easy to derive the amount of bits that can be sent in the next time interval.
%In the LTE radio interface, the unit of allocation, i.e., the PRB, is composed by $12$ subcarriers and $7$ OFDM symbols, and within a single subframe of duration $1$ ms the minimum allocation per user is $2$ PRBs.

\begin{comment}
\begin{equation}
    \sigma_i = \left( \sum_{m}^{M} \Gamma_{m} \pi_{m,i} \right) T_i y_i
\end{equation}
\end{comment}
%$N_{SC}$ defines the number of subcarriers, $N_{OFDM}$ is the number of OFDM symbols,

Traffic demands are compared with the current channel availability to derive the possibilities to pass from one state to another. It must be noticed that the accuracy of the resulting steady-state distribution strictly depends on the precision of such comparison. For this reason, we constantly monitor and update the transition probabilities of the Markov chain based on the resource allocation adopted in the current decision interval. During the arm selection, if the chosen configuration does not provide enough resources to meet the latency requirements, the steady-states will be mostly distributed in the upper part of the Markov chain leading to a minor reward that, in turn, guides the MAB agent to take a different action (i.e., selecting a different arm) in the following decision round.

\begin{figure}[t!]
      \centering
      \includegraphics[trim = 1.5cm 0cm 1cm 0cm , clip, width=0.9\columnwidth]{figures/prbs.pdf}
      \vspace{-3mm}
      \caption{Impact of different resource allocation chunk sizes.}
      \label{fig:prbs}
\end{figure} 

For benchmarking purposes, we implement two widely used MAB algorithms, namely ``legacy'' UCB and Thompson Sampling (TS)\footnote{Due to space limits, we refer the reader to the literature introducing such algorithms, e.g.~\cite{Agrawal2017}.}. On the one hand, UCB adopts a deterministic approach to deal with the exploration-vs-exploitation dilemma, but its performance generally degrades as the number of arms increases. On the other hand, Thompson sampling adopts a probabilistic approach that scales better with the number of arms, but it may provide sub-optimal results when the distribution of reward changes over time (in non-stationary scenarios). Conversely, \name{} combines the advantages of them both by adopting a probabilistic model (MDP) guiding an exploration phase derived from UCB.

We first explore the trade-off between action space (and its granularity) and the associated reward loss. To this aim, we set up a simple experiment with $2$ slices with equal SLA requirements in a deterministic and static environment. We then apply \name{} using $3$ different action sets: $\{0, 2, 4, \dots, 100\}$, $\{0, 5, 10, \dots, 100\}$ and $\{0, 10, 20, \dots, 100\}$ PRBs (with $50$, $20$ and $10$ available configurations each), labeled ``2 PRBs``, ``5 PRBs`` and ``10 PRBs``, respectively. The results, shown in Fig.~\ref{fig:prbs} make it evident that the higher the granularity the longer the exploration phase(s): over $50$ intervals for ``2 PRBs`` whereas it takes around $10$ intervals for ``10 PRBs``. Interestingly, the loss in reward attained to the latter configuration is only $2\%$. Therefore, due to a faster convergence time at the expense of minimal reward loss, we empirically select ``10 PRBs`` granularity for our simulations campaign.

%As expected, the model complexity increases with the granularity of the resource allocation due to the higher number of possible actions (i.e., slice configurations). Fig.~\ref{fig:prbs} shows the algorithm behavior in a static scenario where only $2$ slices are deployed with the same requirements. After a first exploration of all available slice configurations (i.e., available arm in the MAB), the solution tends to select the same configuration (i.e., the configuration that equally assigning the same number of PRBs per slice) that provides the highest revenue. However, as shown in the figure, when the granularity of a selection is $2$ PRBs, there are several possible combinations that exacerbates the complexity of the solution and spreads the actions on different configurations (with similar revenue gains). Increasing the number of PRBs (per configuration) reduces the granularity and, in turn, limits the problem complexity leading the solution to select almost always the same optimal configuration. 

\subsection{Slice SLA violation analysis}

\subsection{Multi-armed bandit problem behavior}
\label{sec:MAB_behaviour}
\begin{figure}[t!]
      \centering
      \includegraphics[trim = 1cm 0cm 1cm 0cm , clip, width=0.9\columnwidth]{Comparison_of_Dropped.pdf}
      \vspace{-4mm}
      \caption{Cumulative dropped traffic due to latency constraints violations.}
      \label{fig:cumulative_dropped}
\end{figure}

We thus grant spectrum-time resources in the granularity of chunks of $1~\text{second}\times10~\text{PRBs}$.
In the first scenario, we investigate the capacity of \name{} to adapt the resource allocation at variable traffic loads. For this reason, we consider only two slices with equal requirements, i.e. ${\nu_i^2}=10$ Mb/s and $\Delta_i=20$ ms for $i={1,2}$. To assess real scenarios with non-stationary traffic patterns, we vary the mean load of each slice $i$ following a  sinusoidal curve in counter-phase between $\mu_i=8$ Mb/s and $\mu_i=40$ Mb/s. This forces the resource allocation process to span across the whole configuration set when dealing with SLAs guarantees. As shown in Fig.~\ref{fig:cumulative_dropped}, the cumulative dropped traffic of each slice changes when different MAB algorithms are used. The behaviour of UCB shows high variability after few decision intervals. As soon as all the arms are selected, the agent starts learning about the statistics of the outcomes and builds a ranked list. The need for a comprehensive knowledge of all the arms leads to several "bad" choices during the exploration phase. This slows down the convergence to the optimal configuration and penalizes performance. From the obtained rewards, TS builds a bivariate probability distribution across the expected reward of each arm, extracts a random sample and chooses the arm associated to the maximum value. This approach performs well in static scenarios as TS favours exploitation of the empirical results obtained in the first attempts; but in time-varying scenario as the one we are considering, the reward distribution associated to each arm fluctuates over time rendering TS unable to adapt fast enough in highly-dynamic scenarios. In contrast, the \name{}'s model-awareness allows for quicker convergence and so it accommodates real-time traffic requirements in dynamic environments and as a result reduces the amount of data violating delay deadlines.

%average reward obtained by the system as function of the number of arms selection, where each line introduces a new slices following Table\ref{tab:slices} \tbd{and others with similar requirements}. The initial behaviour shows high variability in the results due to the UCB exploration phase. As soon as all the arms are selected, the agent starts learning about the statistics of the outcomes and builds a ranked list. The process ends with the finding of the best configuration to be enforced in the next time period.

\begin{figure*}[t!]
    \centering
	  \begin{subfigure}[b]{.32\textwidth}
          \includegraphics[trim = 0cm 0cm 0cm 0cm,clip, width=\linewidth]{figures/2Heatmap.pdf}
          \caption{Effects of different slice requirements.}
          \label{fig:heatmap}
      \end{subfigure}%
	  \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[trim = 0cm 0cm 0cm 0cm, clip,width=\linewidth]{CDFv2.pdf}
        \caption{CDF of experienced latency.}
        \label{fig:cdf}
      \end{subfigure}%
	  \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[trim = 0.5cm 0cm 1.5cm 0cm,clip,width=\linewidth]{figures/regret.pdf}
        \caption{Empirical cumulative regret.}
        \label{fig:cumulative}
      \end{subfigure}%
    \vspace{-2mm}
    %\setlength{\abovecaptionskip}{-1pt} 
    % \setlength{\belowcaptionskip}{-4pt} 
    \caption{\small Effects of different slice requirements (a); CDF of latency experienced by served traffic (b); Empirical cumulative regret for a variable number of slices (c).}
    \vspace{-3mm}
	\label{fig:Sims_results}
\end{figure*}



Obviously, heterogeneous throughput/latency requirements impact the system differently. Fig.~\ref{fig:heatmap} shows the effect of such variations on the system extending the previous scenario and considering increasing values of resource requirements as $10\cdot\alpha$ Mb/s, and $10\cdot\beta$ ms, respectively. As expected, smoother delay requirements (horizontal direction in the figure) allow to serve more traffic within the latency bounds defined by the SLA, although the impact becomes negligible after few incremental steps. This is due to long decision intervals when compared to the timescale of fast channel variations. A proper resource configuration selection allows to match the offered traffic requirements with the expected channel capacity, allowing the incoming traffic to be served within few milliseconds. As the offered traffic approaches the channel capacity boundary (vertical direction in the figure), the same task becomes more challenging and the admission and control process should consider this aspect when granting/rejecting access to new network slices.


\name~'s abilities to adapt to demand variations not only mitigates the amount of traffic violating delay requirements but also improves the distribution of data delivery delay overall. As shown by Fig.~\ref{fig:cdf}, the empirical CDF of delay for each slice in the same scenario presented above remarkably improved with a mean delay equal to $2.6$, $3.9$ and $4.9$ ms for \name{}, TS and UCB, respectively.

Finally, we implement an optimal offline policy with full knowledge of the system, i.e., an oracle policy that knows the future with the corresponding latency violations. We compare both \name{} and TS to this optimal policy for a variable number of slices. The aggregated demand is adapted to ensure we operate within the system capacity. In Fig.~\ref{fig:cumulative}, we depict the temporal evolution of the cumulative reward loss over time (regret) for both approaches. The figure illustrates how the regret increases with time much rapidly for TS, a difference that increases with the number of slices.


%Provided that running slices fit within the admissibility region of the system, Fig.~\ref{fig:cumulative} gives an insight of possible performance drop due to an increasing number of slices and consequent increase of the configuration space. The dashed line represents the outcome of an optimal policy with comprehensive knowledge of the system, i.e. an offline policy able to guarantee that each slice will not be affected by delay in any decision interval. %It worth to highlight again that we assume such a policy exists as heritage of the admission and control engine that allows only slice request with suitable requirements to be admitted. 
%On the one side, it can be noticed that TS’ performance suffer for the increasing number of slices as the complexity of the decision process augments and the relatively lower amount of exploration done by TS misses the chance to select the best instantaneous configuration options. On the other hand, \name{} closely follows the performance of the optimal policy even with an increasing number of slices. 
%With reference to \S~\ref{sect:reward_def} that relates the reward associated to each arm with the delay experienced by the slices, these results confirm that \name{}~assures traffic coming from admitted slices to be served within the boundaries defined by the SLA. 

%leading to performances comparable with the optimal ones. ,

%It worth to highlight again the importance of a proper admission and control engine able to guarantee that only slice request with suitable requirements are admitted in the system.
%Finally, Figure \ref{fig:cumulative} provides an insight on the delay performance as function of an increasing number of slices.
 

==> sections/Related.tex <==
\section{Related Work}
\label{sect:related}

The RAN design problem has always been at the forefront of the mobile operators and a vast amount of research has been devoted to novel RAN architectures~\cite{Rostami, fluidran-jsac} and efficient radio resource schedulers~\cite{lasr, Guo}. Recently, network slicing has been proposed as a new means for mobile operators to deploy isolated network services owned by different customers over a common physical infrastructure. However, as highlighted in~\cite{da2016impact}, RAN needs additional functionalities to fully exploit SDN and NFV principles, specially in the partition and isolation of radio resources. The authors of~\cite{foukas_orion} focus on efficient sharing of the RAN resources and proposed a RAN slicing solution that performs adaptive provisioning and isolation of radio slices. Their work is based on dynamic virtualization of base station resources, which gives tenants the ability to independently manipulate each slice. Although the proposed architecture may guarantee isolation through different control planes, no mechanism is in place to ensure the satisfaction of delay requirements. \cite{mobicom2018_MGFBC} provides an empirical study of resource management efficiency in slicing-enabled networks through real data collected from an operational mobile network, considering different kinds of resources and including radio access, transport and core of the network. Similarly, the authors of~\cite{Chang2018} formulate an optimization framework to deal with resource partitioning problem, where inter-slice isolation is assured through a virtualized layer that decouples the reservation choice from the physical resource availability and proposing different abstraction types of radio resource sharing.

The exploration-vs-exploitation trade-off, typical of Multi-Armed Bandit (MAB) problems is particularly suited to problems that require sequential decision-making. For this reason, a wide set of variations from the classical MAB model has been proposed in the literature~\cite{survery_mab, Mahajan2008}, together with novel algorithms to address them~\cite{Algorithms2000}. In this regard, the work of~\cite{OnlineMAB-Tekin} investigates the MAB problems in case of Markovian reward distribution, where arms change their state in a two-state Markovian fashion. The authors addressed the problem assuming that the Markov chain evolves only when the arm is played, showing that the proposed sample mean-based index policy achieves regret performances comparable to legacy UCB algorithm.
The authors of~\cite{Agrawal2017} performed a complete regret analysis of the TS algorithm, generalizing the original formulation to distributions other than the Beta distribution. 
The MAB framework is also applied in~\cite{Proutiere_sigmetrics18} to deal with rate adaptation problem in 802.11-like wireless systems. The authors demonstrate that exploiting additional observations significantly improve the system performance. Similarly, \cite{Stahlbuhk2018_mobihoc}  deals scheduling transmissions in presence of unknown channel statistics. The proposed algorithm learns the channels' transmission rates while simultaneously exploiting previous observations to obtain higher throughput. This led to the design of a queue-length-based scheduling policy using the channel learning algorithm as a component in time-varying environment.
The authors of~\cite{Hill2017} presented an algorithm for multivariate optimization on large decision spaces based on an innovative approach combining hill climbing optimization and Thompson sampling. While the scalability of their algorithm has been proven through exhaustive simulations, the framework lacks a complete analysis of regret bounds aimed at demonstrating the impact of hill climbing in combinatorial decision making.
Finally, similar to us, \cite{Besbes2014} deals with an MAB formulation where the reward distributions are characterized by temporal uncertainties. Interestingly, they were able  mathematically capture, in terms of reward, the added complexity embedded in the non-stationarity feature when compared to the legacy framework.

The key novelty of our approach, \name, is that it exploits (abstract) information of the underlying system structure to expedite solutions. Conversely, prior works are blind to such type of information and need to spend substantial time exploring very bad decisions before realizing so.


%In ~\cite{Maghsudi2016}, the MAB framework is used to address an energy-efficient resource allocation problem in a 5G ultra-dense scenario, where multiple small-cells need to co-exist over the same radio spectrum. In this scenario, the bandit model allows to select multiple arms in every round, each arm representing a small cell that should be activated in order to improve the overall network performances. Constraints are given in terms of energy consumption.

==> sections/SystemModel.tex <==
\section{\name: The framework overview}
\label{sect:framework}
Our framework solution relies on the concept of slicing-enabled networks wherein multiple network tenants are willing to obtain a network slice with predefined service level agreements (SLAs). Such SLAs may be expressed in terms of maximum slice throughput and average access latency. In particular, we focus on the radio access network (RAN) domain and design \name, a RAN controller that dynamically provisions spectrum resources to admitted network slices while providing latency guarantees. In the following, we overview the main system building blocks with detailed notation and assumptions.

\subsection{Business scenario}
%We envisage the allocation of radio resources towards the end-users as a two-step process. Initially, once network slices are admitted into the system, the infrastructure provider schedules the assignment of slots of radio resources for each of the tenant. The amount of resources assigned depends on the Service Level Agreements (SLAs) occurred during the admission phase. Then, based on the resource availability, each tenant may decide to enforce proprietary scheduling solutions towards its clients, depending on use-case or business requirements
We consider different entities in our system: $i$) an \emph{infrastructure provider} owning the physical infrastructure who offers isolated  RAN slices as a service, $ii$) \emph{tenants} who acquire and manage slices with given SLAs to deliver services to end-users, and $iii$) \emph{end-users}, who demand radio resources from such tenants/slices. 

Let us define $\mathcal{I}$ as the set of running network slices and $\mathcal{U}_i$ as the set of end-users associated to the $i$-th slice. The total amount of wireless resource (radio spectrum) is split into multiple non-overlapping network slices, each one belonging to one single tenant $i\in\mathcal{I}$.\footnote{We assume a one-to-one mapping between slices and tenants. Therefore, we use $i\in\mathcal{I}$ interchangeably throughout the paper as a tenant identifier or its associated slice. Note that this assumption can be relaxed.} Based on fixed SLAs, each network slice is characterized by~\emph{maximum throughput} and \emph{expected latency} denoted by $\Lambda_i$ and $\Delta_i$, respectively. We assume that an admission control process\footnote{Given the plethora of solutions in the literature, the admission control design is out of the scope of this work. We refer the reader, for example, to~\cite{Slicing2018CoNEXT, Sciancalepore2017Optimising} for more details.} is concurrently running on a higher tier so that the mean aggregate load is within the system capacity region. While a slice may be restricted to specific geographical areas, hereafter we assume that a slice is available across the entire system for convenience of notation, but relaxing this assumption is straightforward.

\subsection{Notation} 
We use conventional notation. We let $\mathbb{R}$ and $\mathbb{Z}$ denote the set of real and integer numbers. 
We use $\mathbb{R}_+$, $\mathbb{R}^n$, and $\mathbb{R}^{n\times m}$ to represent the sets of non-negative real numbers, $n$-dimensional real vectors, and  $m\times n$ real matrices, respectively. Vectors are denoted as column vectors and written in bold font. Subscripts represent an element in a vector and superscripts elements in a sequence. For instance, $\langle \vvi x{t} \rangle$ is a sequence of vectors with $\vvi x{t} =   [ x^{(t)}_1, \dots,  x^{(t)}_n   ]^T$ being a vector from $\mathbb{R}^n$, and  $x^{(t)}_i$ the $i$'th component of the $t$'th vector in the sequence. Operation $[\cdot]^T$ represents the transpose operator while $[x_1,\dots,x_n]_{\text{diag}}$ translates the vector into a diagonal matrix. Last, $\vv{\mathbb{1}}$ and $\vv{\mathbb{0}}$  indicate an all-ones and all-zeroes vector, respectively, and $\lceil\cdot\rceil$ is the ceiling operation.
 %and $\vv x \preceq \vv y$ indicates that $x_i \le y_i,

\begin{table}[!ht]
\footnotesize
\centering
\caption{Notation table}
\vspace{-4mm}
\label{tab:notations}
\begin{tabular}{|l|l||l|l|}
\hline
Notation     & Description & Notation  & Description  \\ \hline
$b\in\mathcal{B}$   & base station index & $C_b$ & capacity of $b$ \\
$y_i$ & slice configuration & $i\in\mathcal{I}$ & slice index \\
$n$ & decision epoch index & $r_i^{(n)}$ & bits not served \\
$u_i\in\mathcal{U}_i$ & user index & $\bar{u}_i$ & aggregate user\\
$d\in\{0,1\}$ & exceed delay flag & $g\in\mathcal{G}$ & channel level\\
$\lambda_i^{(n)}$ & inst. traffic demand & $\gamma_i^{(n)}$ & inst. SNR \\ 
$f(x,\rho_i)$ & traffic demands distr. & $f(x,\theta_i)$ & channel distr. \\ 
$\zeta(\cdot)^{(n)}$ & throughput mapping & $\Delta_i$ & latency tolerance\\
$\sigma\in\Sigma$ & MDP state index & $\phi\in\Phi$ & action index\\ 
$w\in\mathcal{W}$ & (latent) channel quality & $\omega(\cdot)$ & latent var. weight\\
$T(\cdot)$ & transition function & $R(\cdot)$ & reward function\\ 
$z_\sigma$ & arm selection freq. & $\psi(\sigma)$ & accuracy value \\ 
$\mathcal{N}_i(\mu_i ,\nu_i^2)$\!\! & Normal distribution & $L_i$ & latency constraint\\
$m\in\mathcal{M}$ & MCS index & $\Gamma_m$ & bits per subframe \\ 
\hline
\end{tabular}
\end{table}
%\end{comment}

\subsection{Problem Definition}
\label{sect:prob_def}
Our system comprises a set of base stations $\mathcal{B}$, where each $b\in\mathcal{B}$ is characterized by a capacity $C_b$, which is the sum of a discrete set of  available physical resource blocks (PRBs) of fixed bandwidth (e.g., 180 kHz in LTE systems). This resource availability must be divided into subsets of PRBs (i.e., slices), and our job is to dynamically assign such subsets to each network slice $i\in\mathcal{I}$. We refer to such assignment as the \emph{configuration} of slice $i$, denoted by the variable $y_i$.
Obviously, we shall guarantee $\sum_{i\in\mathcal{I}} y_i = C_b$, $\forall b\in\mathcal{B}$. For the sake of clarity, we summarize all mathematical variables used throughout the paper in Table~\ref{tab:notations}.

We consider a time-slotted system where time is divided into \emph{decision epochs}\footnote{The decision epoch duration may be decided according to the infrastructure provider policies, ranging from few seconds up to several minutes.} $n = \{ 1,2,\dots\}$. While the admission controller (pre-)selects a subset of slices that can co-exist without exceeding the capacity of the system \emph{in average}, the dynamic nature of the slice's load and wireless channel may cause instantaneous load surges or channel quality fading effects and hence induce a non-zero mean delay. 
%might happen that instantaneous network changes may momentarily impair the network slicing assignment process by delaying traffic packets. 
%
%In particular, this can be caused by the random nature of the wireless channel--due to instantaneous fading and shadowing effects---as well as by the instantaneous slice traffic demand. 
We denote the experienced instantaneous signal-to-noise-ratio (SNR) of slice $i$ (averaged out across all users of the slice) and the instantaneous aggregate traffic demand within time-slot $n$ as $\gamma_i^{(n)}$ and $\lambda_i^{(n)}$, respectively. As each tenant $i$ may show different behavior in terms of wireless channel evolution (according to $\theta_i$) and traffic demands (according to $\rho_i$), we also assume $\gamma_i^{(n)}$ and $\lambda_i^{(n)}$ are drawn from different univariate probability density function, i.e., $\gamma_i^{(n)} \sim f(x,\theta_i)$ and $\lambda_i^{(n)} \sim f(x,\rho_i)$.
%Therefore, we assume $\gamma_i^{(n)}$ and $\lambda_i^{(n)}$ are drawn from different univariate probability density function, i.e., $\gamma_i^{(n)} \sim f(x,\theta_i)$ and $\lambda_i^{(n)} \sim f(x,\rho_i)$, as each tenant $i$ may show different behavior in terms of wireless channel evolution (according to $\theta_i$) and traffic demands (according to $\rho_i$).
Importantly, we do not assume any knowledge on such random variables; we exploit machine learning techniques to \emph{learn} the inherent channel and demand models, which allow our system to dynamically adapt the slice configurations $y_i^{(n)}$ at every decision epoch $n$ while mitigating latency constraint violations. 

Formally, the above-described problem becomes:

\vspace{2mm}\noindent \textbf{Problem}~\texttt{LATENCY-CONTROL}:
\begin{equation*}
\label{pr:latency-control}
\begin{array}{ll}
\text{minimize}   &  \lim\limits_{{N\rightarrow\infty}} \sum\limits_{n=1}^N \mathbb{E}\left [\sum\limits_{i\in\mathcal{I}} r_i^{(n)} \right ]\\
\text{subject to} & \mathbb{E}\left [ \frac{\lambda_i^{(n)}}{\zeta \left(y_i^{(n)},\gamma_i^{(n)} \right)+r_i^{(n)}}\right ]\leq \Delta_i, \quad\forall i\in\mathcal{I};\\
				  & \sum\limits_i y_i^{(n)} \geq C_b, \quad \forall n;\\
				  & y_i^{(n)},r_i^{(n)}\in\mathbb{Z}_+, \quad\forall i\in\mathcal{I};
\end{array}
\end{equation*}
%where $\bar\gamma_i^{(n)}$ and $\bar\lambda_i^{(n)}$ represent the instantaneous SNR (averaged out across the tenant's users) and traffic demand (in bits) measured over decision epoch $n$ while 
where $\zeta(\cdot)^{(n)}$ is a mapping function that returns the number of bits that can be served using the allocated number of PRBs ($y_i^{(n)}$) and the current SNR level $\gamma_i^{(n)}$, as per~\cite[{\S7.1.7}]{TS36.213}. The traffic demand might not be satisfied within a single decision epoch incurring in packet queuing and additional delay. Therefore, in our formulation we introduce $r_i^{(n)}$ as a deficit value indicating the number of bits not served  within the agreed slice latency tolerance $\Delta_i$ during the time-slot $n$ (i.e. dropped). The objective of Problem~\texttt{LATENCY-CONTROL} is hence to find a sequence of $\langle y_i^{(n)} \rangle$ configurations such that the expected total non-served traffic demand is minimized. Hereafter whenever is evident from context, we drop the superscript ${(n)}$ to reduce clutter.

\begin{figure}[t!]
      \centering
      \includegraphics[trim = 3cm 3.25cm 1cm 2cm , clip, width=\linewidth ]{figures/Scenario.pdf}
      \vspace{-6mm}
      \caption{Workflow illustration.}
      \label{fig:building_blocks}
\end{figure}


\subsection{Working flow}

For a given slot $n$, problem~\texttt{LATENCY-CONTROL} can be easily linearized\footnote{Function $\zeta(\cdot)$ can be easily approximated with a linear function by applying piece-wise linearization.} and solved with standard optimization tools. However, this approach may exhibit sub-optimal behavior in future epochs if the statistical distributions of $f(x,\theta_i)$ and $f(x,\rho_i)$ are not stationary. Hence, we propose a novel two-fold approach that: $i$) models channel and traffic demand variations based on previous observations, and $ii$) iteratively applies slice settings towards the goal of honouring SLAs.

Fig.~\ref{fig:building_blocks} depicts the building blocks of our solution. \name{} relies on the concept of Markov Decision Process (MDP) as described in \S\ref{sect:mdp} to decide which configuration $y_i$ should be enforced to all active slices $i$, adapting its choice at every epoch $n$ according to the observed \emph{reward} function that measures the incurred latency. In turn, this information is asymptotically calculated within the \emph{Multi-Tenant Slice Latency Calculation} module by means of a homogeneous Discrete-Time Markov Chain (DTMC), described in \S\ref{sect:MC}. The transition probabilities of such DTMC are updated according to previous observations in the \emph{Monitoring and Prediction of Channel Variations} module, described in \S\ref{sect:monitor}.


%In the following, we introduce a two-stage Markov-based model composed by $i)$ an \emph{internal} Markov Chain (MC) modeling the radio channel transitions as experienced by the different slices' end-users, and $ii)$ an \emph{external} Markov Decision Process (MDP) accounting for the infrastructure provider's need to assign network resources while guaranteeing SLA constraints, which exploits the first stage outcomes to optimize the decision policy.
%whether to schedule the resource assignment for the $i$-th slice
 

\section{DTMC Model}
\label{sect:MC}

Hereafter, we analyze the system dynamics through a  Markov Chain-based (MC) model that computes expected channel conditions and violations on latency tolerance. It should be noted that channel variations and traffic demands are independently obtained according to each slice, thus each DTMC may be treated individually without the need to setup a Markov chain accounting for the overall system configuration. Such global DTMC could anyway be easily obtained as linear combination of the individual DTMCs. For the sake of tractability, we consider a single (virtual) user $\bar{u}_i$  with an aggregate traffic demand resulting from the set of users $u_i\in\mathcal{U}_i$ belonging to slice $i$, as depicted in Fig.~\ref{fig:markov}.\footnote{This assumption can be readily relaxed by considering the convolution of single cumulative distribution functions of every user channel and demand variation~\cite{Antonic:2017:MAI:3093742.3093928}.} We also assume a finite number of channel quality levels $G$, which may bound each instantaneous user channel quality $\gamma_i$. This is a system design choice and allows operators to trade off high accuracy for convergence speed, by ranging from a fine-grained scale (large $G$), e.g. by letting each channel quality level be equal to the modulation and coding scheme (MCSs) as defined in the 3GPP standard document~\cite{TS36.213}, to a coarse-grained scale that may capture the channel variation behaviors with limited accuracy, as detailed in \S\ref{sect:monitor}.

\begin{figure}[t!]
      \centering
      \includegraphics[trim = 4cm 6cm 6cm 4cm, clip, width=0.9\columnwidth ]{figures/Markov_Chain.pdf}
    %   \vspace{-6mm}
      \caption{Radio channel variations as Markov chain.}
      \label{fig:markov}
\end{figure}

Let us consider a discrete-time stochastic process $X_t$\footnote{The time scale $t$ of DTMC state switch is much shorter than the decision epoch $n$ used in the MDP described in \S\ref{sect:mdp}.} that takes values from a finite and discrete state space, which is denoted by $\mathcal{S} = \{S_{0,0}, \dots, S_{g,d}, \dots, S_{G,1} \mid 0\le g \le G, x\in\{0,1\}\}$.\footnote{Each DTMC is defined within a state space $\mathcal{S}^i$. We remove the index $i$ to limit the clutter, as the analysis can be easily extended to any other slice $i$.} In particular, a realization of $X_t$ when visiting state $S_{g,d}$ represents virtual user $\bar{u}_i$ experiencing channel level $g\in\mathcal{G}$ with an associated delay exceeding the one specified by the slice SLA ($d=1$) or otherwise ($d=0$). 
%
When considering wireless channel conditions as Rayleigh distributed, it is common practice to model the variations as a sequential visiting of consecutive states, as the channel does not vary faster than the Markov chain time-slot~\cite{Munos1999}. Hence, we define the probability to improve the user channel condition from level $g$ to level $g+1$ as $p_{g,g+1}$ whereas the probability to get a bad channel from level $g$ to level $g-1$ as $q_{g,g-1}$. Last, given the available physical resource blocks (PRBs) assigned to a particular slice $y_i$, the channel quality level $g$ and the overall traffic demand within the time-slot, we model the probability to incur in delay constraint violation as $m_g$ and the probability to keep the access delay within the agreed bound as $l_g$. This process can be formulated as a two-dimensional DTMC $M := \left (\mathcal{S}, P\right)$, where $P$ denotes the following transition probability:
%, and \textbf{$v$} = [$v_i$] is a row vector describing the initial probability distribution.% of the states.
\begin{equation}\label{eq:trans_prob} P = \left| \begin{array}{ccc}
K_m & M \\
L & K_l \end{array} \right|,
\text{where}~K_{x=\{m,l\}} = \{k_{ij}^{(x)}\}
\end{equation}
\[\text{with}~k_{ij}^{(x)} =  
\begin{cases}
1-p_{i,i+1}-q_{i,i-1}-x_i  & \text{if}~i=j, \\
q_{i,j}  & \text{if}~i=j+1, \\
p_{i,j}  & \text{if}~i=j-1, \\
0  & \text{otherwise};
\end{cases}
\] 
\[\text{and}~M = \{m_{i}\}_{\text{diag}}, L = \{l_{i}\}_{\text{diag}}.
\] 
%
Note that we assume $p_{G,G+1} = q_{1,0} = 0$ and each square block $K_{x=\{m,l\}}, M \text{ and } L$ with $\left [G \times G \right ]$ size so that the square matrix $P$ has dimension $\left[2G \times 2G\right ]$.
%The $S \times S$ matrix denoted by $\mathcal{P}$ is known as the transition probability matrix of the Markov chain. Each value $p_{i,j}$ represents the probability that when in state $i$, the process will make a transition to state $j$. We have that $\mathcal{P}$ must satisfy the following constraints:
%\begin{align}
%&  0 \leq p_{i,j} \leq 1,  &  1 \leq i,j \leq S \label{eq: probability1}\\
%& \sum^S_{j=1} p_{i,j} = 1,  & 1 \leq i \leq S \label{eq: probability2}
%\end{align}
%   
%where Eq.~\ref{eq: probability1} assures non-negative probabilities and Eq.~\ref{eq: probability2} guarantees that the sum of the transition probabilities over all the states does not exceed $1$.
Without loss of generality, we assume that such transition probabilities do not depend on the particular time-slot we are evaluating. Thus, we define our DTMC as a time-homogeneous MC where the process $X_t$ evolves based on $\textbf{$\Pi$}(t) = \textbf{$\Pi$}(0) \textbf{$P$}^t$ where the row vectors \textbf{$\Pi$}$(t)$ and \textbf{$\Pi$}$(0)$ represent the first order state probability distribution at time $n$ and $0$, respectively.
In order to evaluate the long-term behavior of our system, we need to calculate the steady-state probability $\Pi^* = \{\pi_s^*\}$ of being in each of the defined states.
%$\pi_i$ of the system, namely find the probability of being in a certain state $s_i$ after a potentially infinite time horizon
It yields that
\begin{equation}
 \textbf{$\Pi^{*}$} = \lim_{n \to \infty} \textbf{$\Pi$}(t) = \textbf{$\Pi$}(0) \lim_{n \to \infty} \textbf{$P$}^t = \textbf{$\Pi$}(0) \textbf{$P^{*}$}.
 \label{eq:limit}
\end{equation}

%\lz{t or n for time?(discrete or continuous)\\}
\begin{comment}Should the limit in Eq.~\eqref{eq:limit} exist, we have
\begin{equation}
\textbf{$\Pi^{*}$} = \textbf{$\Pi$}(0) \textbf{$P^{*}$}.
\end{equation}
\end{comment}

However, the above-described Markov chain is irreducible, as each state may reach through available paths any other state. Therefore, by stochastic theory, if a Markov chain is irreducible and non-periodic, the steady-state probability distribution \textbf{$\Pi^{*}$} always exists, is unique and is independent from the initial conditions. 

%A state $i$ is said to communicate with $j$ if $p_{i,j} > 0$. In mobile networks, the channel conditions can change very rapidly. Potentially, the channel experienced by the end-users can decay from good to bad conditions within two consecutive time-slots, or recover from unfavorable situations as quickly. We model such transitions assuming that given the current state, it is possible to jump to any other state of the chain in the next time interval. %For this reason, a state $i$ is said to communicate with $j$ if we have $p_{i,j} > 0$ for some time instant $n$. 
%\begin{definition}
%A Markov chain is said to be irreducible if and only if it is composed by states that communicate with any other state within the set $\mathcal{S}$.
%\end{definition}
%Finally, the following theorem assures that the asymptotic behavior of a time-homogeneous and irreducible Markov chain always exists:
%\begin{theorem}
%If a Markov chain is irreducible and non-periodic, the asymptotic distribution \textbf{$\Pi^{*}$} always exists, is unique and is independent from the initial conditions.
%\end{theorem}
%\begin{equation}
%     \pi = \lim_{n \to \infty} v\mathcal{P}^n
%\end{equation}

Recalling the total probability theorem and using Eq.~\eqref{eq:trans_prob}, we calculate the steady-state probability distribution as the solution of the following equations
\begin{equation}
\label{eq:steady_states}
\begin{cases}
    (P^T-\vv{\mathbb{1}}_{\text{diag}})\,\Pi^* & = 0  \\
     \vv{\mathbb{1}}\,\Pi^* & = 1
\end{cases}
\end{equation}
where $\vv{\mathbb{1}}_{\text{diag}}$ is the identity matrix.

\section{\mbox{DTMC Monitoring and Prediction}}
\label{sect:monitor}

The asymptotic behavior of a Markov chain depends on the transition probability matrix $P$, which in turn depends on the stochastic processes of the slice traffic demands and wireless channel variations. While several models have been already defined in the literature to derive such probabilities~\cite{FSMC95}, the latency control objective and the need of an accurate estimation exacerbate the problem and render model-fitting approaches impractical. This brings additional complexity and delay the convergence process to the optimal solution.

We apply the concept of \emph{unsupervised learning} to estimate the transition probabilities based on previous observations. In particular, we rely on the well-known theory of \emph{probabilistic latent variable}~\cite{latent_prob}. Let us consider $w\in\mathcal{W}$ as the stochastic latent variable denoting the current channel quality level. Formally, we redefine the transition probability of the above-described DTMC as
%
\begin{equation}
\rho_{a,b}^g = Pr(X_t = S_{g,b} \mid X_{t-1} = S_{g,a}, g=w)
\end{equation} 
%
that is the probability to move from state $S_{g,a}$ to $S_{g,b}$ when the channel level is exactly $g=w$. To easily understand this, note that $\rho_{0,1}^g = m_g$, $\rho_{1,0}^g = l_g$ whereas $\rho_{0,0}^g$ and $\rho_{1,1}^g$ are the probabilities to stay within the same state $S_{g,0}$ and $S_{g,1}$, respectively. We use an expectation maximization technique to estimate such probabilities. To this aim, we enumerate the transitions between $a$ and $b$ upon $g$ in $h^g_{a,b}$ based on the number of times $X_t$ switches to another state (or stays within the same state) between $t$ and $t+1$.
We then derive the \emph{a posteriori} probability as follows.

\begin{align}
&Pr(g=w\mid X_t=S_{g,b},X_{t-1} = S_{g,a}) = \\ 
&\frac{Pr(X_t=S_{g,b}\mid X_{t-1} = S_{g,a},g=w)Pr(g=w)}{\sum\limits_{z\in\mathcal{W}} Pr(X_t=S_{g,b}\mid X_{t-1} = S_{g,a},g=z)Pr(g=z)},\nonumber
\end{align}
and the likelihood probability as the following

\begin{align}
&Pr(X_t=S_{g,b}\mid X_{t-1}=S_{g,a},g=w) =\\ &\frac{\sum\limits_{g\in\mathcal{G}}h^g_{a,b}Pr(g=w\mid X_t=S_{g,b},X_{t-1}=S_{g,a})}{\sum\limits_{\{\alpha,\beta\}\in \{0,1\}^2} \sum\limits_{g\in\mathcal{G}}h^g_{\alpha,\beta}Pr(g=w\!\!\mid\!\! X_t=S_{g,\beta},X_{t-1}=S_{g,\alpha})}\nonumber
\end{align}

and

\begin{align}
&Pr(g=w) = \\
&\frac{\sum\limits_{\{\alpha,\beta\}\in \{0,1\}^2} h^g_{\alpha,\beta}Pr(g=w\mid X_t=S_{g,\beta},X_{t-1}=S_{g,\alpha})}{\sum\limits_{\{\alpha,\beta\}\in \{0,1\}^2} h^g_{\alpha,\beta}}\nonumber
\end{align}
The above system of equations can be solved using an iterative method that yields $\rho_{a,b}^g$. Finally, we calculate the weight of each latent variable based on a given set of previous observations as per the following equation
\begin{align}
\label{eq:weights}
    &\omega(w\mid \hat{\mathcal{S}}_i) = \frac{\sum_{\{\alpha,\beta\}\in\hat{\mathcal{S}}_i} \rho_{\alpha,\beta}^w}{\sum_{g\in\mathcal{W}}\sum_{\{\alpha,\beta\}\in\hat{\mathcal{S}}_i} \rho_{\alpha,\beta}^g},
\end{align}
where $\hat{\mathcal{S}}_i$ denotes the history of transitions (or lack thereof) across $X_t$ among different states belonging to level $0$ or $1$ in the DTMC depicted in Fig.~\ref{fig:markov}. We can generalize the probability to move from a state wherein the latency is under control $S_{g,0}$ to a state incurring unexpected latency $S_{g,1}$, i.e., exceeding the threshold defined in the slice SLA, using the following expression
%
\begin{equation}
\label{eq:trans_prob_inf}
    \rho_{a,b}\! =\! Pr(X_{t+1}\! =\! S_b| X_{t} = S_a,\hat{\mathcal{S}}_i) =\!\!\! \sum_{w\in\mathcal{W}}\!\omega(w\!\mid\! \hat{\mathcal{S}}_i) \rho_{a,b}^w.
\end{equation}
%
In the next section, we design a control-theory process by means of a Markov Decision Process (MDP) that optimally selects the best slice configuration $y_i$ based on the probability to exceed the access latency constrained by the slice SLA. 

\section{Markov Decision Process}
\label{sect:mdp}
We model the decision problem as a Markov Decision Process (MDP) defined by the set of states $\Sigma = \{\sigma\}$, the set of actions $\Phi=\{\phi\}$, the transition function $T(\sigma,\phi,\sigma')$, and the reward function $R(\sigma,\phi)$.
The set of states accounts for all the radio resource splitting options among different tenants, namely \emph{slicing configuration} $c_\sigma=\{y_1,y_2,\dots,y_i,\dots,y_I\}$ expressed in terms of PRBs, where $\sum_{i\in\mathcal{I}}y_i = C$, i.e., the overall capacity is exactly split between running slices. We assume that each slicing configuration is issued at every decision epoch $n$.
The transition function characterizes the dynamics of the system from state $\sigma$ to state $\sigma'$ through action $\phi$. Analytically, $P(\sigma' \mid \sigma,\phi)$ is the probability to visit state $\sigma'$ given the previous visited state $\sigma$ and the action $\phi$.
Finally, the function $R(\sigma,\phi)$ measures the reward associated to the transition from the current state $\sigma$ performing action $\phi$.
%At each step, the system can be influenced by taking one of the possible action $a \in \mathcal{A}$. 
%According to the chosen action, the system earns the associated reward $R(\sigma,\phi)$, and the next state follows based on $T(q,a,\'q)$. 
We shall consider an MDP with an infinite time horizon. Future rewards will be discounted by a factor $0<\beta<1$ to ensure the total reward obtained is finite.

%while the transition time is defined by T (s; a).

When dealing with MDPs is common practice to define a ``policy'' for the decision agent, namely a function $\mathcal{P}^{(n)}: \Sigma^{(n)} \to \Phi^{(n)}$ that specifies which action $\phi$ to perform at time $n$ when in state $\sigma$. As soon as the Markov decision process is combined with a defined policy, this automatically fixes the next action for each state so that the resulting combination exactly behaves similarly to a Markov chain.
%In presence of stochastic processes, a common way to rank a policy with respect to the others is through the measurement, over a potentially infinite time horizon, of the total expected reward. In our case, the reward can be defined as:
%
%\begin{equation}
%    \tbd{ G = \sum_{n=0}^{\infty} R(q_n,\theta(q_n), \pi)}
%    \label{eq:reward}
%\end{equation}
%
%It must be noticed that the reward associated to each state of the MDP depends on the asymptotic probabilities $\pi$ of the first stage Markov chain, linking the two models.
%
%Given the probabilities of being in a certain channel condition, i.e., a state of the MC, it is possible to derive for each slice the expected capacity associated to that channel. 
%In this way, the infrastructure provider can plan, for each decision period, how share the radio resources among the different slices. For example, 
%it may exploit the fact that better channel conditions allow to serve higher throughput with less PRBs utilization, and shrink the resource assignment on those slices that experience very good channel qualities and do not have high throughput requirements, or, it may decide to dedicate spare resources to those slices which, on average, are experiencing disrupted channel conditions in order to respect the SLA agreements.
%
%
%
%We define the value function $V_\theta(q)$ as the expected return starting from state $q$, and then following the policy $\theta$:
%
%\begin{equation}
    %V_\theta(q) = \mathbb{E}_\theta [ G | q ]
%\end{equation}
%
%and the optimal value function $V_{\theta}^{*}(q)$ as the maximum value function over all policies:
%
%\begin{equation}
%  V_{\theta}^{*}(q) = \max_\theta V_{\theta}(q)
%\end{equation}
% 
The final aim of the decision agent is to find the policy that maximizes the expected total reward, or, equivalently, to discover the policy $\mathcal{P}^*$ that maximizes the value function. %The following theorem assures that such a policy exists for every Markov decision process:

%\begin{theorem}
%For any Markov decision process there exists an optimal policy $\theta^{*}$ that provides better or equal value function results with respect to all other policies.
%\end{theorem}

%\tbd{\cite{Auer}}

\subsection{Reward Definition}
\label{sect:reward_def}

Each state (or slicing configuration) is associated with a reward value that influences the agent during the decision process. The rationale behind is that we need to bind the action reward to the probability to exceed the latency constraints defined in the slice SLA. In the following, we introduce the reward function used in our experiments with a detailed overview of its behavior.

Given a slicing configuration $c_\sigma=\{y_i \mid i\in\mathcal{I} \}$, we can analytically build a Discrete-Time Markov Chain, as described in \S\ref{sect:MC}. If the associated transition probability matrix $P$ is perfectly known, we can also derive the steady-state probabilities $\Pi^*=\{\pi_s^*\}$ to be within any single state using Eq.~\eqref{eq:steady_states}. Thus, we can compute the probability to have the access latency of our system under control. This can be used to formulate the instantaneous reward value $R(\sigma^{(n)},\phi^{(n)})$ as
\begin{equation} \label{eq:reward}
    R(\sigma^{(n)},\phi^{(n)}) = \left(\sum_{s\in\mathcal{S}_g,0} \pi^*_s\right)^\eta
\end{equation}
where $s$ is the index of all states $S_{g,0}, \forall g\in\mathcal{G}$ such that the slice latency is under control, whereas $\eta\in [0,1]$ is an adjustable value decided by the infrastructure provider to provide action fairness in the reward function when $\eta$ tends to $0$, or maximum likelihood of keeping latency under control when $\eta$ tends to $1$. Then our objective is to maximize the expected aggregate reward obtained as $\lim\limits_{{N\rightarrow\infty}} \sum\limits_{n=1}^N \mathbb{E}\left[\beta^n R\left(\sigma^{(n)},\phi^{(n)}\right) \right]$. However, given the fully-connected structure of our Markov Decision Process, i.e., all states are reachable from any MDP state, our objective is equivalent to maximize the instantaneous reward given by~\eqref{eq:reward} at each decision epoch $n$.

Nonetheless, the assumption of perfect knowledge on the transition probability matrix $P$ might be not realistic. Therefore, we need to rely on the transition probabilities $\rho_{a,b}$ inferred based on the previous observations, as explained in \S\ref{sect:monitor}, Eq.~\eqref{eq:trans_prob_inf}. The larger the set of observations, the higher the accuracy of our probability estimation and the higher the reward attained to the instantaneous best action taken by the MDP.

\subsection{Complexity analysis}

Once defined all possible states, actions and rewards of our MDP, we can use the Value Iteration algorithm~\cite{valueiteration} to explore the entire MDP and select the optimal state, i.e., the slicing configuration $\sigma$ that returns the best rewards, or equivalently, the configuration that keeps the overall slice latency under control. Value Iteration needs to keep track of all visited states and rewards in order to optimally guide the decision process. The overall number of states might be very large and must be investigated.

Let us assume that $I$ slices are active and running in our system. Also, assume that each slice configuration $y_i$ can take values from a discrete set of chunks of $10$ PRBs ranging from $0$ to $C$. Assuming that the slicing configuration must be consistent, i.e., $\sum_{i\in\mathcal{I}}y_i = C$, we can calculate the overall number of states equal to $\frac{(C+I-1)!}{(I-1)!C!}$.
This results in the well known \emph{curse of dimensionality} problem, which compromises scalability especially when the number of running slices is high. Therefore, in the next section we rely on an online technique to reduce the complexity of our approach while still attaining near-optimal results.
%An infrastructure provider must take into consideration those numbers when planning the resource allocation. A too conservative reservation policy might cause resource wastage, while one strictly related at the current utilization might induce SLA violations when mixed with unfavorable channel conditions. If the resource reservation policy applied in this decision interval does not guarantee the transmission of $\lambda_i$, the exceeding amount of bits $\Delta_i = \sigma_i - \lambda_i$ are
%of bits that does not fit into the current channel reservation will be 
%postponed to a subsequent transmission interval, incurring in additional delay. The overall experienced delay will depend on traffic flows characteristics, channel conditions and also on resource reservation policies applied in the next decision intervals. %The infrastructure provider should in first place define an allocation policy that avoids resource under provisioning, and in second place, compensate for channel


\subsection{Multi-armed Bandit problem}
\label{sect:mabmodel}

The online decision-making problem has been addressed in the past with several mathematical tools~\cite{survery_mab}. The limited information about real-time channel quality and effective traffic demand forces the operator to choose, like a gambler facing diverse options to play, the number of radio resources to assign to each running slice. This automatically falls in the fundamental \emph{exploration-vs-exploitation} dilemma: the gambler needs to carefully balance the exploitation operations on known slicing configurations that provided the best revenues in the past against the exploration of new slicing configuration that might eventually produce higher revenues.

This class of decision process can be captured by a Multi-Armed Bandit (MAB) problem formulation, which emulates the action of selecting the best (single) bandit (or slot machine) that may return the best payoff. Each slot machine returns unpredictable revenues out of fixed statistical distribution, not known \emph{a priori}, that is iteratively inferred by previous observations. This matches well the randomness of the channel quality and the traffic demand we aim to capture whereas each bandit can be mapped onto a state of the MDP, i.e., a specific slicing configuration. The final objective of such a problem is to maximize the overall gain after a finite number of rounds. This class of problems is usually assessed by a defined metric called \emph{regret} $\Omega$, which is defined as the difference between the reward that can be gained by an optimal oracle, i.e., using an optimal policy that knows the reward distributions \emph{a priori}, and the expected reward of the myopic online policy.

Reusing notation from our MDP model, let us define each arm $\sigma \in \Sigma$ as a different slicing configuration $c_\sigma = \{y_i \mid i \in\mathcal{I}\}$. Once selected, each arm provides an instantaneous reward $R(\sigma)$ defined as the following
\begin{equation}\label{eq:classic_mab_reward}
    R(\sigma) = \sum_{i\in\mathcal{I}}\left(\zeta(y_i,\gamma_i)-\frac{\lambda_i}{\Delta_i}\right)
\end{equation}
where the slicing configuration is $y_i\in c_\sigma$, $\zeta(\cdot)$ computes the number of bits that can be served using $y_i$ configuration and given the current channel quality $\gamma_i$, and $\lambda_i$ is the slice traffic demand, as described in \S\ref{sect:prob_def}.

While using such reward function requires low overhead, as it only needs to calculate the incurred latency after selecting a slicing configuration, it only converges to a near-optimal solution after exploring several configurations, which results in overly long training periods (as shown in \S\ref{sect:perf_eval}). This is an inherent issue with classic MAB methods, which are \emph{blind} to the underlying system structure. Conversely, in this paper we resort to a novel model-assisted approach that exploits the system model of \S\ref{sect:reward_def} to guide the exploration/exploitation process with (abstract) system information. In this way, as opposed to using the traditional reward model of Eq.~\eqref{eq:classic_mab_reward}, we define our bandit's reward as the expectation of access latency exceeding slice SLA defined in Eq.~\eqref{eq:reward}. This has a two-fold advantage: $i$) during the initial training period, the DTMC associated to each state of the MDP is updated (and enhanced) with more accurate values of the transition probabilities: this helps to find steady-state probabilities (and in turn an updated reward per slicing configuration) that reflect the real behavior of our system as time goes on; and $ii$) the slicing configuration selection accounts directly for stochastic behaviors of both channel quality and traffic demand, while reducing the state space to those that may benefit the entire system.

Many algorithms have been proposed to optimally solve the MAB while learning from previous observations~\cite{Vermorel2005}. One of the main issues is that collecting rewards on a short-time basis may negatively impact on the decision of the best bandit. Thus, we rely on a modified version of the so-called \emph{Upper Confidence Bound} (UCB) algorithm devised by~\cite{AuerMab2002} that overcomes this issue by measuring not only the rewards collected up to the current time interval, but also the \emph{confidence} in the reward distribution estimations by keeping track of how many times each bandit has been selected $z_{\sigma,n}$. The pseudo-code is listed in Algorithm~\ref{alg:ucb}.

\begin{algorithm}[t!]
\caption{\small{\textbf{\name{}}}}
\label{alg:ucb}
\algsetup{indent=1em}
\begin{footnotesize}
\begin{algorithmic}[1]
\STATE {\bf Input: }$ \Sigma, N, \Psi =\{\psi(\sigma)\}$
\STATE {\bf Initialization: }$  z_{\sigma},\hat{\rho}_{\sigma} = 0,\,\,\forall \sigma$
\STATE {\bf Procedure:}
\FORALL {$n \in N$}
\IF {$n = 0$} \label{line}
    \FORALL {$\sigma \in \Sigma$}
    \STATE GET reward: $\hat{\rho}_{\sigma}=  R_{\sigma}^{(n)}$
    \STATE $z_{\sigma} = z_{\sigma} + 1$
    \ENDFOR
\ELSE
	\STATE $\sigma^* = \argmax\limits_{\sigma\in\Sigma}\hat{\rho}_{\sigma} + \psi(\sigma) \sqrt{\frac{2\log{\sum_k z_{k}} }{z_{\sigma}}}$
	\STATE UPDATE $\hat{\rho}_{\sigma^*} \leftarrow R_{\sigma^*}^{(n)}$
	\STATE $z_{\sigma} = z_{\sigma} + 1$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{footnotesize}
\end{algorithm}

 Initially, we explore all bandits, i.e., slicing configuration $\sigma\in\Sigma$, to get a consistent reward (line 2-6). Then we select the best configuration that maximizes the empirical distribution $\hat\rho_\sigma$ accounting for a confidence value. This confidence value depends on the number of times we have explored that particular configuration as well as the accuracy of the transition probabilities we calculate for the associated DTMC. Note that this is different to traditional UCB algorithms. Specifically, we define a Markov accuracy value $\psi(\sigma) = (\frac{(\sum_w \omega(w\mid\hat{\mathcal{S}}_i))^2}{W\sum_{w}\omega(w\mid\hat{\mathcal{S}}_i)^2})$ that depends on the weights $\omega(\cdot)$ based on the performed observations $\hat{\mathcal{S}}_i$, as reported in Eq.~\eqref{eq:weights}. Interestingly, $\psi(\sigma)\in(0,1]$, i.e., when the DTMC has no relevant observations to build its transition probabilities this function returns $\psi(\sigma) =1$ whereas, when a relevant number of observations allows to determine accurate transition probabilities, this value tends to $0$.


\subsection{Regret analysis}
Here, we mathematically calculate the bounds of our solution, \name, for multi-armed bandit problems. Let us consider a player selecting an arm $\sigma\in\Sigma$ every decision epoch $n$. Every time arm $\sigma$ is pulled down, it returns a reward $R_{\sigma}^{(n)}$ drawn from an unknown distribution with mean $\bar{\rho}_\sigma$ and empirical mean value calculated until time $n$ as $\hat{\rho}_{\sigma}^{(n)}=\frac{\sum_{s=1}^n R_{\sigma}^{(s)}}{n}$. We denote $\sigma^*$ as the arm providing the maximum average reward such that $\bar{\rho}_{\sigma^*}>\bar{\rho}_\sigma, \forall\sigma\neq\sigma^*$.
If the arm selection is performed using \name, it yields that the regret is obtained as
\begin{align} \label{eq:regret}
\Omega_N^{\text{\name{}}}(\Sigma) & = N\bar{\rho}_{\sigma^*}-\mathbb{E}[\sum\limits_{n=1}^NR_{\sigma}^{(n)}\mid \sigma\in\mathcal{P}^{\text{\name{}}}] \nonumber\\
				  & = N\bar{\rho}_{\sigma^*}-\sum\limits_{\sigma=1}^{\Sigma} \bar{\rho}_{\sigma} \mathbb{E}[z_{\sigma}^{(n)}];
\end{align}
where $\mathcal{P}^{\text{\name{}}} = \{{\sigma_n}\}$ is the policy as defined in \S\ref{sect:mdp} that consists of a set of moves that \name{} will play at time $n$ whereas $z_{\sigma,n}$ is the overall number of decision epochs arm $\sigma$ has been pulled down till time instant $n$. Now consider \name{} as a uniformly good policy, i.e., any suboptimal arm $\sigma\neq{\sigma^*}$ is chosen by our policy up to round $n$ so that $\mathbb{E}[z_{\sigma,n}] = o(n^\alpha),\forall \alpha>0$. It holds that
\begin{equation}
\lim_{\text{N}\to\infty} \sum\limits_{\sigma=1}^{\Sigma} N^{-1}\bar{\rho_\sigma} \mathbb{E}[z_{\sigma}^{(N)}] = \Sigma \bar{\rho}_{\sigma^*}. 
\end{equation}
Hence, we can express the regret lower bound as the following
\begin{equation}
\lim_{\text{N}\to\infty}\inf \frac{\Omega_N^{\text{\name{}}}(\Sigma)}{\log N} \geq \!\!\!\!\sum\limits_{\sigma:\,\, \bar{\rho}_\sigma<\bar{\rho}_{\sigma^*}} \!\frac{\bar{\rho}_{\sigma^*}-\bar{\rho}_{\sigma}}{Div(\bar{\rho}_\sigma,\bar{\rho}_{\sigma^*})}
\end{equation}
where $Div(\bar{\rho}_\sigma,\bar{\rho}_{\sigma^*})$ is the Kullback-Leibler divergence of one statistical distribution against the other and it is used to measure how one distribution might diverge from another probability distribution.

Now consider the Hoeffding's inequality for multiple i.i.d. variables $x_n$ with mean $\mu$. It yields that $Pr(|\frac{\sum_{i=1}^n x_i}{n}-\mu|\geq\delta)\leq 2e^{-2n\delta^2}$. Our algorithm \name{} applies an upper confidence interval $\delta = \sqrt{\frac{2\log\sigma_kz_k}{z_\sigma}}$. Therefore, it yields that
\begin{equation}
    Pr\left(|\hat{\rho}_{\sigma,n}-\bar{\rho}_\sigma|<\sqrt{\frac{2\log\sum_kz_k}{z_{\sigma}}}\right) \geq 1-\frac{2}{t^4}
\end{equation}
and also that
\begin{equation}
    Pr\left(\mathcal{P}^{(n+1)}=\sigma\mid z_{\sigma}^{(n)}>\frac{4\log n}{\bar{\rho}_{\sigma^*}-\bar{\rho}_{\sigma}}\right) \leq \frac{4}{t^4}.
\end{equation}
We can then derive the expectation of number of times sub-optimal arm $\sigma\neq{\sigma^*}$ is pulled down as follows
\begin{equation}
    \mathbb{E}[z_{\sigma}^{(N)}] \leq \frac{4\log N}{\bar{\rho}_{\sigma^*}-\bar{\rho}_{\sigma}}+8
\end{equation}
and the regret upper bound as the following
\begin{equation}
    \mathbb{E}\left[\Omega_N^{\text{\name{}}}(\Sigma)\right]\leq \sum\limits_{\sigma:\,\, \bar{\rho}_\sigma<\bar{\rho}_{\sigma^*}}\frac{4\log N}{\bar{\rho}_{\sigma^*}-\bar{\rho}_{\sigma}}+8\left(\bar{\rho}_{\sigma^*}-\bar{\rho}_{\sigma}\right).
\end{equation}

%Adverse radio channel conditions may lead to a drop of traffic performance metrics, and consequent SLA latency violations.
%Let us consider, for example, the transmission of a constant traffic flow with average throughput requirements $\Lambda_k$ under the settings defined by the generic slice $k$, as depicted in Fig.~\ref{fig:latency}.
%At time $n_1$, the radio channel conditions are good enough to support both the flow transmission and the latency requirements, thus there are no problem in satisfying the SLA. At time $n_2$, radio interference occurs and the channel quality experienced by the end-user drops. In LTE networks, this event is reported back to the base station by means of Channel Quality Indicator (CQI) messages~\cite{TS36.213}. Such information forces the local scheduler in the base station to reduce the assigned Modulation and Coding Scheme (MCS) for that specific user, finally leading to a decrease of the throughput performances. At this point, the channel conditions do not allow to transmit at the agreed slice-rate $\Lambda_k$ anymore, nor the traffic can satisfy the delay requirements, potentially leading to SLA violations. In order to recover from this situation and guarantee the \emph{average} satisfaction of the requirements, in the next decision interval more radio resources should be dedicated to slice $k$.



==> sections/abstract.tex <==
\begin{abstract}

%XC The technical specification of the next generation of mobile networks, namely 5G networks, has been recently released bringing together new business requirements and emerging technology initiatives.
%XC In particular, such technological means give prominence to the concept of \emph{network slicing}, commonly understood as the ability of a 5G infrastructure owner to provide, via virtualization, a subset of network and computational resources to different tenants so as to build (virtual) vertical services or Mobile Virtual Network Operator (MVNOs) systems.
\emph{Network Slicing} is expected to become a game changer in the upcoming 5G networks and beyond, enlarging the telecom business ecosystem through still-unexplored vertical industry profits.
This implies that heterogeneous service level agreements (SLAs) must be guaranteed \emph{per slice} given the multitude of predefined requirements. 

In this paper, we pioneer a novel radio slicing orchestration solution that simultaneously provides \emph{latency} and {throughput} guarantees in a multi-tenancy environment. Leveraging on a solid mathematical framework, we exploit the exploration-vs-exploitation paradigm by means of a multi-armed-bandit-based (MAB) hierarchical orchestrator, \name, that makes adaptive resource slicing decisions with no prior knowledge on the traffic demand or channel quality statistics. As opposed to traditional MAB methods that are blind to the underlying system, \name{} relies on system structure information to expedite decisions. 

After a preliminary simulations campaign empirically proving the validness of our solution, we implement \name{} in off-the-shelf equipment that fully emulate realistic network conditions: near-optimal results within affordable computational time are measured when \name{} is in place.
\end{abstract} 

==> sections/conclusion.tex <==
\section{Conclusions}
\label{sect:concl}

Major efforts in the design of next-generation mobile systems pivot around network slicing and (mobile edge) low-latency services. This paper aims to bridge the gap between them both by designing \name, a RAN-specific network slice orchestrator that considers network slice requests with \emph{strict latency requirements}. Despite the efforts devoted by 5G researchers and engineers to network slicing, to the best of our knowledge, this is the first radio slicing mechanism that provides \emph{formal delay guarantees}. 

To make network slicing decisions in environments with varying wireless channel quality and user demands, \name{} builds on a learning Multi-Armed Bandit (MAB) method that is \emph{model-aware} as opposed to classic MAB approaches that are blind to information regarding the underlying system. In addition, we exploit information from the system model to expedite the exploration-vs-exploitation process. Our results derived from an implementation with off-the-shelf hardware show that \name{} is able to guarantee strict slice latency requirements at affordable computational costs.

==> sections/introduction.tex <==


The quest for new sources of revenue that revitalizes the mobile industry has spawned an unprecedented hype around the fifth-generation of mobile networks (5G) and, in particular, the network slicing concept. Enabled by software-defined networking (SDN) and network function virtualization (NFV), network slicing allows telco operators to offer virtualized slices of infrastructure resources \emph{on-demand} to heterogeneous 3${^{\text{rd}}}$-party services~\cite{WhitePaperMWC}. %XC Remarkably, the inertia of industry has fostered substantial standardization effort~\cite{TS23.501, NGMN2016SlicingConcept} and academic research work~\cite{Sciancalepore2017Optimising,foukas_orion}.
%, network slicing can allocate (virtual) infrastructure resources to different \emph{instances} of network slices in an isolated manner, and accommodate in this way multiple heterogeneous services (associated to different tenants) under a common physical infrastructure. %XC Remarkably, the inertia of industry has fostered substantial standardization effort~\cite{TS23.501, NGMN2016SlicingConcept} and academic research work~\cite{Sciancalepore2017Optimising,foukas_orion}. 
A high-level view of the system considered in this paper is described in Fig.~\ref{fig:slicing}. The figure represents a series of \emph{sliceable} base stations as a pool of radio resources (coloured cubes in the figure). The resource allocation process is considered hierarchical: while \emph{bundles} of radio resources are assigned to different tenants (namely radio slices), each tenant autonomously schedules its bundle of radio resources to each individual user following classic radio scheduling policies. The difference between such operations is subtle but of paramount importance: a slice controller operates at a larger timescale and thus a coarser granularity~\cite{Slicing2018CoNEXT, foukas_orion}. 

Given the plethora of works on classic radio scheduling~\cite{Sharma,Lee}, we keep this aspect out of the scope of this paper and we focus instead on the former impelling need: a proper design of an orchestration solution that autonomously assigns chunks of radio spectrum (slices) in relatively larger time-scales pursuing the goal of \emph{guaranteeing simultaneously latency and throughput constraints}. From the best of our knowledge, there is a non-negligible lack of works focusing on both aspects simultaneously in sliced-network environments. 
While most prior work on network slicing focuses on average bit-rate guarantees~\cite{foukas_orion, Sciancalepore2017Optimising}, \emph{latency} considerations have received little attention.
However, a novel solution is required to face with advanced use-cases requirements that might include low-latency constraints and throughput guarantees, e.g. for autonomous driving and platooning~\cite{Lee2018_lowlatency} in V2X-enabled scenarios.

\begin{figure}[t!]
      %\vspace{-2mm}
      \centering
      \includegraphics[trim = 2cm 5cm 5cm 1cm, clip, width=\linewidth ]{figures/network_slicing.pdf}
      \vspace{-8mm}
      \caption{\small Illustration of the network slicing concept.}
      \label{fig:slicing}
      %\vspace{-2mm}
\end{figure}

To fill this gap, we design a LAtency-Controlled Orchestrator (\name{}), a network slice controller that maps virtual radio resource allocations to physical resources while still guaranteeing latency requirements\footnote{Note that \name{} does \emph{not} compete with state-of-the-art throughput-only slice controllers---in fact, we purposely assume the presence of an admission controller that ensures that the aggregate load incurred by granted slices is within the system capacity region.}. Specifically, \name{} augments such prior work by accommodating resources to (granted) slices such that latency agreements are satisfied. This unlocks a new business opportunity for the telco operators
that may apply customized pricing models according to the \emph{elasticity} of offered slice latency constraints.
%We also note that, while \name~assigns chunks of radio resources to tenants, we assume the presence of a per-tenant scheduler that ultimately allocates virtual radio resources to individuals that belong to the tenant's network. 

{\bf Technical challenges.} While designing \name{}, two sources of uncertainty need to be under control: $i$) the behavioral dynamics of the (aggregated) demand across involved tenants and $ii$) the inherent randomness of the wireless channel. These system dynamics have been traditionally modeled via either complex models that are hard to solve in realistic settings or via simplistic assumptions at the expense of low performance figures. In our work, we explore a novel approach by designing a scheme that \emph{learns} the implications that allocation decisions have on per-slice latency without explicitly making assumptions on the underlying dynamics. To this aim, we first model our decision-making problem as a Markov Decision Process\footnote{With a little misuse of nomenclature, we will refer to Markov Decision Process (MDP) rather than Semi-Markov Decision Process (SMDP) despite considering continuous time scales.} (MDP), which allows us to neglect low-level details of the tenant demands and channel dynamics while letting us retain some knowledge on the consequences that a given action might have on the most immediate next system state. 

An MDP model helps us to fully explore the problem features. However, the process of learning the state transition probability matrix of each of the embedded Markov chains incurs in prohibitive overhead as a reinforcement learning agent has to explore the whole space of state-action trajectories---the so-called \emph{the curse of dimensionality}. To address this, we resort to a Multi-Armed Bandit (MAB) model where the attained reward depends only on the action taken from a bounded set of possible actions. Importantly, in contrast to traditional MAB methods, \name{} is \emph{model-aware} (though not model-dependant), i.e., it exploits (abstracted) information regarding the underlying system to expedite the selection of highly rewarding actions, which is particularly attractive when dealing with dynamic non-stationary scenarios. %XC Conversely, traditional methods are blind to the system structure and hence require exploring bad decisions far too long.

In summary, the main contributions of our paper can be summarized as follows:
\begin{itemize}
    \item We introduce a Discrete-Time Markov Chain (DTMC) model to capture the dynamics of the (instantaneous) aggregate slice traffic demand and the wireless channel variations;
    \item We present a latent variable regression model to accurately anticipate the transition probability matrix of the proposed DTMCs;
    \item We formulate the dynamic slice resource provisioning as a Markov Decision Process (MDP);
    \item We design a \emph{model-aware} Multi-Armed Bandit (MAB) method to guide the decision-making process, which relies on the above DTMC models and anticipated transition probabilities to speed up convergence;
    \item We present an exhaustive simulations campaign to preliminary assess the performance of our approach.
    \item We fully implement and field-test our solution using off-the-shelf equipment that emulate real network conditions: \name{} shows its innovative performance gain against considered legacy techniques.
\end{itemize}

The remainder of the paper is structured as follows. \S\ref{sect:framework} formulates our problem and presents the main building blocks of \name{}. \S\ref{sect:MC} introduces an DTMC model that helps us expedite the action-space exploration phase and \S\ref{sect:monitor} deeply analyzes it. In \S\ref{sect:mdp}, we introduce our decision process as a Markov Decision Process (MDP) and present a model-aware Multi-Armed Bandit decision-making engine integrated in \name{}. \S\ref{sect:perf_eval} presents our preliminary simulation campaign to validate the design principles of \name{}, whereas \S\ref{sect:poc} details the implementation of our novel solution into off-the-shelf equipment with realistic network performance. Finally, \S\ref{sect:related} summarizes related literature and \S\ref{sect:concl} concludes the paper with some final remarks.


%In \S\ref{sect:framework} we provide an overall view of our framework, namely \name{}, detailing the problem formulation and the main building blocks. In \S\ref{sect:MC}, we summarize our findings on the stochastic processes related to the instantaneous slice traffic demand and the channel variation, and we model them as a Discrete-Time Markov Chain (DTMC). In \S\ref{sect:monitor}, we provide insights on how to iteratively adjust the transition probabilities of the DTMC based on the previous observations. In \S\ref{sect:mdp}, we introduce our decision process as a Markov Decision Process (MDP) and we show that the Multi-Armed Bandit solution best fits our formulation. In \S\ref{sect:perf_eval}, we carry out an exhaustive simulations campaign to prove the validness of our novel framework while in \S\ref{sect:related} we evaluate the state-of-the-art. Finally, we provide our concluding remarks in \S\ref{sect:concl}.

%We envisage the allocation of radio resources towards the end-users as a two-step process. Initially, once network slices are admitted into the system, the infrastructure provider schedules the assignment of slots of radio resources for each of the tenant. The amount of resources assigned depends on the Service Level Agreements (SLAs) occurred during the admission phase. Then, based on the resource availability, each tenant may decide to enforce proprietary scheduling solutions towards its clients, depending on use-case or business requirements.

%The infrastructure provider needs to define a suitable reservation policy for its network in order to satisfy the tenants request. This introduces a fundamental trade-off: a too aggressive reservation policy may save resources allowing to admit more slice requests in the future increasing the final revenues, while a too conservative one might cause resource wastage.
%Moreover, channel conditions may vary within two consecutive decision interval leading to violation of the SLAs.

